The classification of frequencies in the {\gamma} Doradus / {\delta} Scuti hybrid star HD 49434

Hybrid stars of the {\gamma} Doradus and {\delta} Scuti pulsation types have great potential for asteroseismic analysis to explore their interior structure. To achieve this, mode identi- fications of pulsational frequencies observed in the stars must be made, a task which is far from simple. In this work we begin the analysis by scrutinizing the frequencies found in the CoRoT photometric satellite measurements and ground-based high-resolution spectroscopy of the hybrid star HD 49434. The results show almost no consistency between the frequencies found using the two techniques and no characteristic period spacings or couplings were identified in either dataset. The spectroscopic data additionally show no evidence for any long term (5 year) variation in the dominant frequency. The 31 spectroscopic frequencies identified have standard deviation profiles suggesting multiple modes sharing (l, m) in the {\delta} Scuti frequency region and several skewed modes sharing the same (l, m) in the {\gamma} Doradus frequency region. In addition, there is a clear frequency in the {\gamma} Doradus frequency region that appears to be unrelated to the others. We conclude HD 49434 remains a {\delta} Scuti/ {\gamma} Doradus candidate hybrid star but more sophisticated models dealing with rotation are sought to obtain a clear picture of the pulsational behaviour of this star.

==> bib.tex <==
\clearpage
\bibliographystyle{mn2e}
\bibliography{references}
 

==> subfigure.tex <==
%%
%% This is file `subfigure.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% subfigure.dtx  (with options: `package')
%% 
%% Copyright (C) 1986-2002 Steven Douglas Cochran.
%% 
%% This file is NOT the source for subfigure, because almost all comments
%% have been stripped from it.  It is NOT the preferred form of subfigure
%% for making modifications to it.
%% 
%% Therefore you can NOT redistribute and/or modify THIS file.  You can
%% however redistribute the complete source (subfigure.dtx and
%% subfigure.ins) and/or modify it under the terms of the LaTeX Project
%% Public License, either version 1.2 of this license or (at your option)
%% any later version. The latest version of this license is in:
%%      http://www.latex-project.org/lppl.txt
%% and version 1.2 or later is part of all distributions of LaTeX version
%% 1999/09/03 or later.
%% 
%% The subfigure package is distributed in the hope that it will be
%% useful, but WITHOUT ANY WARRANTY; without even the implied warranty of
%% MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the LaTeX
%% Project Public License for more details.
%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% @LaTeX-style-file{
%%    author     = "Steven Douglas Cochran",
%%    version    = "2.1.5",
%%    date       = "2005/04/29",
%%    time       = "14:24:08",
%%    filename   = "subfigure.sty",
%%    address    = "Digital Mapping Laboratory, School of Computer Science
%%                  Carnegie-Mellon University, 5000 Forbes Avenue
%%                  Pittsburgh, PA 15213-3890, USA",
%%    telephone  = "+1 412.268.5654",
%%    fax        = "+1 412.268.5576",
%%    email      = "cochran@ieee.org",
%%    codetable  = "ISO/ASCII",
%%    keywords   = "LaTeX, float, figure, table, captcont",
%%    supported  = "yes",
%%    abstract   = "LaTeX package for providing support for the
%%                  inclusion of small, `sub', figures and tables.  It
%%                  simplifies the positioning, captioning and
%%                  labeling of them within a single figure or table
%%                  environment.  In addition, this package allows
%%                  such subcaptions to be written to the List of
%%                  Figures or List of tables if desired."
%% }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\NeedsTeXFormat{LaTeX2e}[1994/12/01]
\ProvidesPackage{subfigure}[2002/03/15 v2.1.5 subfigure package]
\def\sf@floatfix#1#2{%
  \ifx#1#2%
    \ifx#1\@undefined\else
      \PackageWarningNoLine{subfigure}{%
Your document class has a bad definition^^J
of \string#1, most likely^^J
\string\let\string#1=\string#2^^J
which has now been changed to^^J
\string\def\string#1{\string#2}^^J
because otherwise subsequent changes to \string#2^^J
(like done by several packages changing float behaviour)^^J
can't take effect on \string#1.^^J
Please complain to your document class author}%
      \def#1{#2}%
    \fi
  \fi}
\begingroup
\def\next#1#2{%
    \endgroup
  \sf@floatfix\endfigure{end@float}
  \sf@floatfix\endtable\end@float
  \sf@floatfix#1\end@dblfloat
  \sf@floatfix#2\end@dblfloat}
\expandafter\next\csname endfigure*\expandafter\endcsname
  \csname endtable*\endcsname
\newif\ifhyperrefloaded
\AtBeginDocument{%
  \@ifpackageloaded{hyperref}{%
    \hyperrefloadedtrue
    \providecommand\theHsubfigure{\thefigure.\arabic{subfigure}}%
    \providecommand\theHsubtable{\thetable.\arabic{subtable}}%
    \providecommand{\toclevel@subfigure}{1}%
    \providecommand{\toclevel@subtable}{1}}{}}
\newif\ifsubcaphang
\newif\ifsubcapcenter
\newif\ifsubcapcenterlast
\newif\ifsubcapnooneline
\newif\ifsubcapraggedright
\newskip\subfigtopskip     \subfigtopskip    =  5\p@
\newskip\subfigcapskip     \subfigcapskip    =  0\p@
\newdimen\subfigcaptopadj  \subfigcaptopadj  =  3\p@
\newskip\subfigbottomskip  \subfigbottomskip =  5\p@
\newdimen\subfigcapmargin  \subfigcapmargin  =  \z@
\newskip\subfiglabelskip   \subfiglabelskip  =  0.33em plus 0.07em minus 0.03em
\newcommand*{\subcapsize}{}
\newcommand*{\subcaplabelfont}{%
  \subcaplabelfont@f\subcaplabelfont@c\subcaplabelfont@s}
\newcommand*{\subcaplabelfont@f}{\fontfamily{\familydefault}\selectfont}
\newcommand*{\subcaplabelfont@c}{\fontseries{\seriesdefault}\selectfont}
\newcommand*{\subcaplabelfont@s}{\fontshape{\shapedefault}\selectfont}
\newcommand*{\subcapfont}{%
  \subcapfont@f\subcapfont@c\subcapfont@s}
\newcommand*{\subcapfont@f}{\fontfamily{\familydefault}\selectfont}
\newcommand*{\subcapfont@c}{\fontseries{\seriesdefault}\selectfont}
\newcommand*{\subcapfont@s}{\fontshape{\shapedefault}\selectfont}
\newif\ifsf@tight          \sf@tighttrue
\newcounter{subfigure}[figure]
\@ifundefined{figuretopcaptrue}{\newif\iffiguretopcap}{}
\newif\ifsubfiguretopcap
\let\p@subfigure=\thefigure
\providecommand*{\thesubfigure}{(\alph{subfigure})}
\renewcommand*{\thesubfigure}{(\alph{subfigure})}
\newcommand*{\@thesubfigure}{\thesubfigure\hskip\subfiglabelskip}
\newcommand*{\@@thesubfigure}{\thesubfigure}
\let\ext@subfigure=\ext@figure
\newcommand*{\l@subfigure}{%
  \@dottedxxxline{\ext@subfigure}{2}{3.8em}{2.5em}}
\newcounter{lofdepth}
\setcounter{lofdepth}{1}
\newcounter{subtable}[table]
\@ifundefined{tabletopcaptrue}{\newif\iftabletopcap}{}
\newif\ifsubtabletopcap
\let\p@subtable=\thetable
\providecommand*{\thesubtable}{(\alph{subtable})}
\renewcommand*{\thesubtable}{(\alph{subtable})}
\newcommand*{\@thesubtable}{\thesubtable\hskip\subfiglabelskip}
\newcommand*{\@@thesubtable}{\thesubtable}
\let\ext@subtable=\ext@table
\newcommand*{\l@subtable}{%
  \@dottedxxxline{\ext@subtable}{2}{3.8em}{2.5em}}
\newcounter{lotdepth}
\setcounter{lotdepth}{1}
\DeclareOption{normal}{%
  \subcaphangfalse
  \subcapcenterfalse
  \subcapcenterlastfalse
  \subcapnoonelinefalse
  \subcapraggedrightfalse}
\DeclareOption{hang}{\subcaphangtrue}
\DeclareOption{center}{\subcapcentertrue}
\DeclareOption{centerlast}{\subcapcenterlasttrue}
\DeclareOption{nooneline}{\subcapnoonelinetrue}
\DeclareOption{raggedright}{\subcapraggedrighttrue}
\DeclareOption{isu}{\ExecuteOption{hang}}
\DeclareOption{anne}{\ExecuteOption{centerlast}}
\DeclareOption{scriptsize}{\renewcommand*{\subcapsize}{\scriptsize}}
\DeclareOption{footnotesize}{\renewcommand*{\subcapsize}{\footnotesize}}
\DeclareOption{small}{\renewcommand*{\subcapsize}{\small}}
\DeclareOption{normalsize}{\renewcommand*{\subcapsize}{\normalsize}}
\DeclareOption{large}{\renewcommand*{\subcapsize}{\large}}
\DeclareOption{Large}{\renewcommand*{\subcapsize}{\Large}}
\DeclareOption{rm}{\renewcommand*{\subcaplabelfont@f}{\rmfamily}}
\DeclareOption{sf}{\renewcommand*{\subcaplabelfont@f}{\sffamily}}
\DeclareOption{tt}{\renewcommand*{\subcaplabelfont@f}{\ttfamily}}
\DeclareOption{md}{\renewcommand*{\subcaplabelfont@c}{\mdseries}}
\DeclareOption{bf}{\renewcommand*{\subcaplabelfont@c}{\bfseries}}
\DeclareOption{up}{\renewcommand*{\subcaplabelfont@s}{\upshape}}
\DeclareOption{it}{\renewcommand*{\subcaplabelfont@s}{\itshape}}
\DeclareOption{sl}{\renewcommand*{\subcaplabelfont@s}{\slshape}}
\DeclareOption{sc}{\renewcommand*{\subcaplabelfont@s}{\scshape}}
\DeclareOption{RM}{\renewcommand*{\subcapfont@f}{\rmfamily}}
\DeclareOption{SF}{\renewcommand*{\subcapfont@f}{\sffamily}}
\DeclareOption{TT}{\renewcommand*{\subcapfont@f}{\ttfamily}}
\DeclareOption{MD}{\renewcommand*{\subcapfont@c}{\mdseries}}
\DeclareOption{BF}{\renewcommand*{\subcapfont@c}{\bfseries}}
\DeclareOption{IT}{\renewcommand*{\subcapfont@s}{\itshape}}
\DeclareOption{SL}{\renewcommand*{\subcapfont@s}{\slshape}}
\DeclareOption{SC}{\renewcommand*{\subcapfont@s}{\scshape}}
\DeclareOption{UP}{\renewcommand*{\subcapfont@s}{\upshape}}
\DeclareOption{figbotcap}{\figuretopcapfalse}
\DeclareOption{figtopcap}{\figuretopcaptrue}
\DeclareOption{tabbotcap}{\tabletopcapfalse}
\DeclareOption{tabtopcap}{\tabletopcaptrue}
\DeclareOption{FIGBOTCAP}{\ExecuteOptions{figbotcap}\subfiguretopcapfalse}
\DeclareOption{FIGTOPCAP}{\ExecuteOptions{figtopcap}\subfiguretopcaptrue}
\DeclareOption{TABBOTCAP}{\ExecuteOptions{tabbotcap}\subtabletopcapfalse}
\DeclareOption{TABTOPCAP}{\ExecuteOptions{tabtopcap}\subtabletopcaptrue}
\DeclareOption{loose}{%
  \subfigtopskip    = 10\p@
  \subfigcapskip    = 10\p@
  \subfigcaptopadj  =  0\p@
  \subfigbottomskip = 10\p@
  \subfigcapmargin  = 10\p@
  \subfiglabelskip  =  0.33em
  \renewcommand*{\@thesubfigure}{\thesubfigure\space}
  \renewcommand*{\@thesubtable}{\thesubtable\space}
  \sf@tightfalse}
\DeclareOption{tight}{%
  \subfigtopskip    =  5\p@
  \subfigcapskip    =  0\p@
  \subfigcaptopadj  =  3\p@
  \subfigbottomskip =  5\p@
  \subfigcapmargin  =  \z@
  \subfiglabelskip  =  0.33em plus 0.07em minus 0.03em
  \renewcommand*{\@thesubfigure}{\thesubfigure\hskip\subfiglabelskip}
  \renewcommand*{\@thesubtable}{\thesubtable\hskip\subfiglabelskip}
  \sf@tighttrue}
\ExecuteOptions{normal,footnotesize,FIGBOTCAP,TABBOTCAP,loose}
\InputIfFileExists{subfigure.cfg}{%
  \typeout{****************************************^^J%
           * Local config file subfigure.cfg used *^^J%
           ****************************************}}{}
\ProcessOptions
\newcommand*{\subfigure}{%
  \bgroup
    \let\subfig@oldlabel=\label
    \let\label=\subfloat@label
    \@nameuse{if\@captype topcap}\else
      \advance\@nameuse{c@\@captype}\@ne
    \fi
    \refstepcounter{sub\@captype}%
    \@ifnextchar [%
      {\@subfigure}%
      {\@subfigure[\@empty]}}
\let\subtable=\subfigure
\def\@subfigure[#1]{%
    \@ifnextchar [%
      {\@subfloat{sub\@captype}[{#1}]}%
      {\@subfloat{sub\@captype}[\@empty{#1}][{#1}]}}
\newskip\subfig@top
\newskip\subfig@bottom
\long\def\@subfloat#1[#2][#3]#4{%
    \@tempcnta=1
    \ifsf@tight
      \if@minipage
        \@tempcnta=\z@
      \else\ifdim \lastskip=\z@ \else
        \@tempcnta=2
      \fi\fi
    \fi
    \@nameuse{if\@captype topcap}%
      \subfig@top=\subfigbottomskip
      \subfig@bottom=\subfigtopskip
    \else
      \subfig@top=\subfigtopskip
      \subfig@bottom=\subfigbottomskip
    \fi
    \leavevmode
    \setbox\@tempboxa \hbox{#4}%
    \@tempdima=\wd\@tempboxa
    \vtop\bgroup
      \vbox\bgroup
        \ifcase\@tempcnta
          \@minipagefalse
        \or
          \vspace{\subfig@top}%
        \or
          \ifdim \lastskip=\z@ \else
            \@tempskipb\subfig@top\relax\@xaddvskip
          \fi
        \fi
        \@nameuse{if#1topcap}%
          \ifx \@empty#3\relax \else
            \@subcaption{#1}{#2}{#3}%
            \vskip\subfigcapskip
            \vskip\subfigcaptopadj
          \fi\egroup
          \box\@tempboxa
        \else
          \box\@tempboxa\egroup
          \ifx \@empty#3\relax \else
            \vskip\subfigcapskip
            \@subcaption{#1}{#2}{#3}%
          \fi
        \fi
      \vspace{\subfig@bottom}%
    \egroup
    \@nameuse{if\@captype topcap}\else
      \global\advance\@nameuse{c@\@captype}\m@ne
    \fi
  \egroup}
\newcommand*{\@subfigcaptionlist}{}
\newcommand{\@subcaption}[3]{%
  \ifx \relax#2\relax \else
    \bgroup
      \let\label=\@gobble
      \let\protect=\string
      \def\@subcaplabel{\@nameuse{@@the#1}}%
      \xdef\@subfigcaptionlist{%
        \@subfigcaptionlist,%
        {\protect\numberline{\@subcaplabel}\noexpand{\ignorespaces #2}}}%
    \egroup
  \fi
  \@nameuse{@make#1caption}{\@nameuse{@the#1}}{#3}}
\newcommand*{\listsubcaptions}{%
  \@ifstar
    {\gdef\@subfigcaptionlist{}}%
    {\@listsubcaptions{\@captype}}}
\newcommand*{\@listsubcaptions}[1]{%
  \@ifundefined{@captype}{}{%
    \@ifundefined{ext@sub#1}{}{%
      \@for \sf@temp:=\@subfigcaptionlist \do {%
        \ifx \@empty\sf@temp\relax \else
          \addcontentsline
            {\@nameuse{ext@sub#1}}%
            {sub#1}%
            {\sf@temp}%
        \fi}}}%
  \gdef\@subfigcaptionlist{}}
\newcommand{\@makesubfigurecaption}[2]{%
  \setbox\@tempboxa\hbox{%
    \subcapsize
    {\subcaplabelfont #1}%
    {\subcapfont\ignorespaces #2}}%
  \@tempdimb=-\subfigcapmargin
  \multiply\@tempdimb\tw@
  \advance\@tempdimb\@tempdima
  \hbox to\@tempdima{%
    \hss
    \ifdim \wd\@tempboxa >\@tempdimb
      \subfig@caption{#1}{#2}%
    \else\ifsubcapnooneline
      \subfig@caption{#1}{#2}%
    \else
      \box\@tempboxa
    \fi\fi
    \hss}}
\let\@makesubtablecaption=\@makesubfigurecaption
\newcommand{\subfig@caption}[2]{%
  \ifsubcaphang
    \sbox{\@tempboxa}{\subcapsize\subcaplabelfont #1}%
    \addtolength{\@tempdimb}{-\wd\@tempboxa}%
    \usebox{\@tempboxa}%
    \subfig@captionpar{\@tempdimb}{%
      {\subcapfont\ignorespaces #2}}%
  \else
    \subfig@captionpar{\@tempdimb}{%
      {\subcaplabelfont #1}%
      {\subcapfont\ignorespaces #2}}%
  \fi}
\newcommand{\subfig@captionpar}[2]{%
  \parbox[t]{#1}{%
    \subcapsize
    \ifsubcapraggedright
      \setlength{\leftskip}{\z@}%
      \setlength{\@rightskip}{\@flushglue}%
      \setlength{\rightskip}{\@rightskip}%
      \setlength{\parindent}{\z@}%
    \else\ifsubcapcenter
      \setlength{\leftskip}{\@flushglue}%
      \setlength{\rightskip}{\@flushglue}%
      \setlength{\parfillskip}{\z@skip}%
    \else\ifsubcapcenterlast
      \addtolength{\leftskip}{\z@ plus 1fil}%
      \addtolength{\rightskip}{\z@ plus -1fil}%
      \setlength{\parfillskip}{\z@ plus 2fil}%
    \fi\fi\fi
    #2}}
\newcommand*{\@dottedxxxline}[6]{%
  \ifnum #2>\@nameuse{c@#1depth}\else
    \@dottedtocline{0}{#3}{#4}{#5}{#6}
  \fi}
\let\subfig@end@float=\end@float
\renewcommand*{\end@float}{%
  \@listsubcaptions{\@captype}%
  \subfig@end@float}
\let\subfig@end@dblfloat=\end@dblfloat
\renewcommand*{\end@dblfloat}{%
  \@listsubcaptions{\@captype}%
  \subfig@end@dblfloat}
\let\subfig@oldcaption=\@caption
\long\def\@caption#1[#2]#3{%
  \@ifundefined{if#1topcap}%
    {\subfig@oldcaption{#1}[{#2}]{#3}}%
    {\@nameuse{if#1topcap}%
       \@listsubcaptions{#1}%
       \subfig@oldcaption{#1}[{#2}]{#3}%
     \else
       \subfig@oldcaption{#1}[{#2}]{#3}%
       \@listsubcaptions{#1}%
     \fi}}
\let\subfig@oldlabel=\relax
\newcommand*{\subfloat@label}{%
  \@ifnextchar(
    {\sf@sub@label}
    {\sf@sub@label(Sub\@captype\space
                   \@ifundefined{thechapter}{}{%
                     \@nameuse{thechapter}\space}%
                   \@nameuse{p@sub\@captype}%
                   \@nameuse{thesub\@captype}.)}}
\let\sub@label\subfloat@label
\def\sf@sub@label(#1)#2{%
  \ifhyperrefloaded
    \protected@edef\@currentlabelname{%
      \expandafter\strip@period #1\relax.\relax\@@@}%
  \fi
  \sf@@sub@label{#2}}
\newcommand*{\sf@@sub@label}[1]{%
  \@bsphack
  \subfig@oldlabel{#1}%
  \ifhyperrefloaded
    \protected@write\@auxout{}{%
        \string\newlabel{sub@#1}%
            {{\@nameuse{@@thesub\@captype}}%
            {\thepage}%
            {\expandafter\strip@period\@currentlabelname\relax.\relax\@@@}%
            {\@currentHref}%
            {}}}%
  \else
    \protected@write\@auxout{}{%
        \string\newlabel{sub@#1}%
            {{\@nameuse{@@thesub\@captype}}%
            {\thepage}}}%
  \fi
  \@esphack}
\newcommand\subref[1]{%
  \ref{sub@#1}}
\newcommand\Subref[1]{%
  {\subcaplabelfont
   \ref{sub@#1}}}
\endinput
%%
%% End of file `subfigure.sty'.

